Telescoping Filter: A Practical Adaptive Filter

Filters are fast, small and approximate set membership data structures. They are often used to filter out expensive accesses to a remote set S for negative queries (that is, a query x not in S). Filters have one-sided errors: on a negative query, a filter may say "present" with a tunable false-positve probability of epsilon. Correctness is traded for space: filters only use log (1/\epsilon) + O(1) bits per element. The false-positive guarantees of most filters, however, hold only for a single query. In particular, if x is a false positive of a filter, a subsequent query to x is a false positive with probability 1, not epsilon. With this in mind, recent work has introduced the notion of an adaptive filter. A filter is adaptive if each query has false positive epsilon, regardless of what queries were made in the past. This requires "fixing" false positives as they occur. Adaptive filters not only provide strong false positive guarantees in adversarial environments but also improve performance on query practical workloads by eliminating repeated false positives. Existing work on adaptive filters falls into two categories. First, there are practical filters based on cuckoo filters that attempt to fix false positives heuristically, without meeting the adaptivity guarantee. Meanwhile, the broom filter is a very complex adaptive filter that meets the optimal theoretical bounds. In this paper, we bridge this gap by designing a practical, provably adaptive filter: the telescoping adaptive filter. We provide theoretical false-positive and space guarantees of our filter, along with empirical results where we compare its false positive performance against state-of-the-art filters. We also test the throughput of our filters, showing that they achieve comparable performance to similar non-adaptive filters.

==> diagrams/block_diagram.tex <==
% Block diagram
% Sizes
\newcommand{\gridwidth}{30pt}
\newcommand{\gridheight}{15pt}
\newcommand{\gap}{0.2cm}


% Colors
\newcommand{\colorzero}{darkgray!50!lightgray!30!white}
\newcommand{\colorone}{green!50!lightgray!30!white}
\newcommand{\colortwo}{blue!50!lightgray!30!white}
\newcommand{\colorthree}{red!50!lightgray!30!white}
\newcommand{\colorfour}{yellow!50!lightgray!30!white}

\tikzstyle{slot} = [draw, minimum width=\gridwidth, minimum height=\gridheight]

% Single Block in Memory diagram
\begin{figure*}[h]
  \caption{A single block in memory in the \AQF with metadata bits and selectors.}
  \centering
  \begin{tikzpicture}

    % Remainders
    \node (Remainders) at (0, {4*(\gridheight+\gap)}) [left] {Remainders};
    \foreach \x[count = \i from 1] in { a, b, c, d, e, f, 0, h } {
      \node (rem\i) [base right={\gap + \gridwidth*(\i-1)} of Remainders, slot] {\strut\x};
    }

    % Quotients
    \foreach \x[count = \i from 1] in { 0, 1, 2, 3, 4, 5, 6, 7 } {
      \node (quot\i) [above=\gap of rem\i), slot, draw=white!60] {\x};
    }
    \node [base left = \gap of quot1] {Quotients};

    % Occupieds
    \foreach \x[count = \i from 1]/\color in {
      0/white,
      1/\colorone,
      0/white,
      1/\colortwo,
      1/\colorthree,
      0/white,
      0/white,
      1/\colorfour} \node (occ\i) [below=\gap of rem\i, fill=\color, slot] {\strut\x};
    \node [left = \gap of occ1] {Occupieds};

    % Runends
    \foreach \x[count = \i]/\color in {
      1/white,
      0/\colorzero,
      1/\colorone,
      0/white,
      1/\colortwo,
      1/\colorthree,
      0/white,
      1/\colorfour} {
      \node (runend\i) [below=\gap of occ\i, fill=\color, slot] {\strut\x};
    }
    \node [left = \gap of runend1] {Runends};

    % Selectors
    \node (sels) [below={\gap*2 + \gridheight} of runend1.west, 
                  anchor=west, draw, 
                  minimum width={\gridwidth*7}] {\strut 1618649850735163};
    \node [left = \gap of sels] {Encoded Selectors};

    % Offset
    \node (offset) [right=-\pgflinewidth of sels.east, draw, 
                    minimum width={\gridwidth},
                    fill=\colorzero] {\strut 1};
    \node (Offset) [right = \gap of offset] {Offset};

  \end{tikzpicture}\label{fig:blocks}
\end{figure*}


==> diagrams/interpretation_diagram.tex <==
% Block interpretation diagram

\begin{figure}[h]
  \caption{Block interpretation: Quotients and Remainders.}
  \centering
  \begin{tikzpicture}
    \node (quotient) at (0,0) [left] {\bfseries\underline{Quotient}};
    \node (remainders) [right=\gridwidth of quotient] {\underline{\bfseries Remainder\tiny (Selector)}};

    % Quotients and remainder
    \node (rem1) [below={\gap + \gridheight} of quotient.west, anchor=west, slot] {Previous Block};
    \node (o) [right=\gridwidth of rem1, slot, fill=\colorzero] {a\tiny 0};
    \draw [->, thick] (rem1) -- (o);

    \foreach \rems[count = \quot-1 from 0]/\color in {
      {}/white,
      {b/0,c/1}/\colorone,
      {}/white,
      {d/0,e/1}/\colortwo,
      {f/0}/\colorthree,
      {}/white,
      {}/white,
      {h/2}/\colorfour}{
      \node (rem1) [below=\gap of rem1, slot] {\quot};
      \xdef\lastx{1}
      \foreach \x[count = \i from 2]/\sel in \rems {
	\node (rem\i) [right=\gridwidth of rem\lastx, slot, fill=\color] {\x\tiny\sel};
	\draw [->, thick] (rem\lastx) -- (rem\i);
	\xdef\lastx{\i};
      }
    }
  \end{tikzpicture}\label{fig:interpretation}
\end{figure}


==> diagrams/selectors_diagram.tex <==
% Selectors interpretation diagram

\newcommand{\gridwidth}{30pt}
\newcommand{\gridheight}{15pt}
\newcommand{\gap}{0.2cm}

\tikzstyle{slot} = [draw, minimum width=\gridwidth, minimum height=\gridheight]
\setlength{\belowcaptionskip}{15pt plus 3pt minus 2pt} % Add space between caption and fig

\begin{figure*}[h]
  \caption{An example of using integer-based arithmetic coding to encode a binary string.}
    \centering
    %FIXME I think this math is wrong
    \begin{tikzpicture}
    \def\sels{ 0, 0, 1, 0, 1 };
    
      \node (label) at (0,0) [anchor=west] 
      {Bitarray};
      \foreach \x[count = \i from 1] in \sels {
        \node [base right={\gap + \gridwidth*(\i-1)} of label, slot] {\x};
        \node (col\i) [below={\gap + (\gap+\gridheight)*(\i-1)} of label] {\strut\x}; 
      }
  
  		\node (beg1) [right={\gridwidth*0} of col1] {};
		\node (end1) [right={\gridwidth*56/8} of col1] {};
		\node (r) [right={\gridwidth*8}of col1] {};
		\draw [dashed] (col1) -- (r);
		\draw [|-|, thick] (beg1) node (b) [below left] {} -- (end1) node (e) [below right] {\tiny$0 + \lfloor\frac78 \cdot 255\rfloor=223$};
  		
  		\node (beg) [right={\gridwidth*0} of col2] {};
		\node (end) [right={\gridwidth*49/8} of col2] {};
		\node (r) [right={\gridwidth*8}of col2] {};
		\draw [dashed] (col2) -- (r);
		\draw [|-|, thick] (beg) node (b) [below left] {} -- (end) node (e) [below right] {\tiny$0 + \lfloor\frac78 \cdot 223 \rfloor=195$};
  		
  		\node (beg) [right={\gridwidth*36/8} of col3] {};
  		\node (end) [right={\gridwidth*47/8} of col3] {};
  		\node (r) [right={\gridwidth*8}of col3] {};
  		\draw [dashed] (col3) -- (r);
  	    \draw [|-|, thick] (beg) node (b) [below left] {\tiny$0 + \lceil\frac78 \cdot 195  \rceil =171$} -- (end) node (e) [below right] {\tiny$171 + \lfloor\frac78 (195-171)\rfloor = 192$};
  	    
  	    \node (beg) [right={\gridwidth*36/8} of col4] {};
  	    \node (end) [right={\gridwidth*46/8} of col4] {};
  	    \node (r) [right={\gridwidth*8}of col4] {};
  	    \draw [dashed] (col4) -- (r);
  	    \draw [|-|, thick] (beg) node (b) [below left] {\tiny$171$} -- (end) node (e) [below right] {\tiny$171 + \lfloor\frac78 \cdot (192-171) \rfloor=189$};
  	    
  	    \node (beg) [right={\gridwidth*43/8} of col5] {};
  	    \node (end) [right={\gridwidth*45/8} of col5] {};
  	    \node (r) [right={\gridwidth*8}of col5] {};
  	    \draw [dashed] (col5) -- (r);
  	    \draw [|-|, thick] (beg) node (b) [below left] {\tiny$171 + \lceil\frac78 \cdot (189-171)  \rceil =187$} -- (end) node (e) [below right] {\tiny$187 + \lfloor\frac78 (189-187)\rfloor = 188$};
  		
  		\node (label) [below={\gap + (\gap+\gridheight)*6} of label.west, anchor=west] 
  		{Final Encoding:};
  		\node (label) [right=\gap of label, slot] 
  		{187};

    \end{tikzpicture}
  \label{fig:selectors}
\end{figure*}

